Haptic Feedback Improves Human-Robot Agreement and User Satisfaction in Shared-Autonomy Teleoperation

Shared autonomy teleoperation can guarantee safety, but does so by reducing the human operator's control authority, which can lead to reduced levels of human-robot agreement and user satisfaction. This paper presents a novel haptic shared autonomy teleoperation paradigm that uses haptic feedback to inform the user about the inner state of a shared autonomy paradigm, while still guaranteeing safety. This differs from haptic shared control, which uses haptic feedback to inform the user's actions, but gives the human operator full control over the robot's actions. We conducted a user study in which twelve users flew a simulated UAV in a search-and-rescue task with no assistance or assistance provided by haptic shared control, shared autonomy, or haptic shared autonomy. All assistive teleoperation methods use control barrier functions to find a control command that is both safe and as close as possible to the human-generated control command. For assistive teleoperation conditions with haptic feedback, we apply a force to the user that is proportional to the difference between the human-generated control and the safe control. We find that haptic shared autonomy improves the user's task performance and satisfaction. We also find that haptic feedback in assistive teleoperation can improve the user's situational awareness. Finally, results show that adding haptic feedback to shared-autonomy teleoperation can improve human-robot agreement.

==> preamble/compactLists.tex <==
% set compact lists
\setlist[1]{\labelindent=\parindent}
\setlist[1]{topsep=3pt, itemsep=-1pt}


==> preamble/graphLocalization.tex <==
% This file was generated by the scriptgenerateGraphLocalization
% Do not modify this file directly

% Notation for nodes
\newcommand{\Ri}{R_{i}}
\newcommand{\dRi}{\dot{R}_{i}}
\newcommand{\ddRi}{\ddot{R}_{i}}
\newcommand{\Ti}{T_{i}}
\newcommand{\dTi}{\dot{T}_{i}}
\newcommand{\ddTi}{\ddot{T}_{i}}

\newcommand{\Rj}{R_{j}}
\newcommand{\dRj}{\dot{R}_{j}}
\newcommand{\ddRj}{\ddot{R}_{j}}
\newcommand{\Tj}{T_{j}}
\newcommand{\dTj}{\dot{T}_{j}}
\newcommand{\ddTj}{\ddot{T}_{j}}


% Notation for edges
\newcommand{\Rij}{R_{ij}}
\newcommand{\Tij}{T_{ij}}
\newcommand{\betaij}{\beta_{ij}}
\newcommand{\cij}{c_{ij}}
\newcommand{\dij}{d_{ij}}
\newcommand{\qij}{q_{ij}}
\newcommand{\lij}{\lambda_{ij}}
\newcommand{\varphiij}{\varphi_{ij}}
\newcommand{\gij}{g_{ij}}

\newcommand{\Rji}{R_{ji}}
\newcommand{\Tji}{T_{ji}}
\newcommand{\betaji}{\beta_{ji}}
\newcommand{\cji}{c_{ji}}
\newcommand{\dji}{d_{ji}}
\newcommand{\qji}{q_{ji}}
\newcommand{\lji}{\lambda_{ji}}
\newcommand{\varphiji}{\varphi_{ji}}
\newcommand{\gji}{g_{ji}}


% Notation for edges, measured quantities
\newcommand{\tRij}{\tilde{R}_{ij}}
\newcommand{\dtRij}{\dot{\tilde{R}}_{ij}}
\newcommand{\tTij}{\tilde{T}_{ij}}
\newcommand{\dtTij}{\dot{\tilde{T}}_{ij}}
\newcommand{\tbetaij}{\tilde{\beta}_{ij}}
\newcommand{\dtbetaij}{\dot{\tilde{\beta}}_{ij}}
\newcommand{\tcij}{\tilde{c}_{ij}}
\newcommand{\dtcij}{\dot{\tilde{c}}_{ij}}
\newcommand{\tdij}{\tilde{d}_{ij}}
\newcommand{\dtdij}{\dot{\tilde{d}}_{ij}}
\newcommand{\tqij}{\tilde{q}_{ij}}
\newcommand{\dtqij}{\dot{\tilde{q}}_{ij}}
\newcommand{\tlij}{\tilde{\lambda}_{ij}}
\newcommand{\dtlij}{\dot{\tilde{\lambda}}_{ij}}
\newcommand{\tvarphiij}{\tilde{\varphi}_{ij}}
\newcommand{\dtvarphiij}{\dot{\tilde{\varphi}}_{ij}}
\newcommand{\tgij}{\tilde{g}_{ij}}
\newcommand{\dtgij}{\dot{\tilde{g}}_{ij}}

\newcommand{\tRji}{\tilde{R}_{ji}}
\newcommand{\dtRji}{\dot{\tilde{R}}_{ji}}
\newcommand{\tTji}{\tilde{T}_{ji}}
\newcommand{\dtTji}{\dot{\tilde{T}}_{ji}}
\newcommand{\tbetaji}{\tilde{\beta}_{ji}}
\newcommand{\dtbetaji}{\dot{\tilde{\beta}}_{ji}}
\newcommand{\tcji}{\tilde{c}_{ji}}
\newcommand{\dtcji}{\dot{\tilde{c}}_{ji}}
\newcommand{\tdji}{\tilde{d}_{ji}}
\newcommand{\dtdji}{\dot{\tilde{d}}_{ji}}
\newcommand{\tqji}{\tilde{q}_{ji}}
\newcommand{\dtqji}{\dot{\tilde{q}}_{ji}}
\newcommand{\tlji}{\tilde{\lambda}_{ji}}
\newcommand{\dtlji}{\dot{\tilde{\lambda}}_{ji}}
\newcommand{\tvarphiji}{\tilde{\varphi}_{ji}}
\newcommand{\dtvarphiji}{\dot{\tilde{\varphi}}_{ji}}
\newcommand{\tgji}{\tilde{g}_{ji}}
\newcommand{\dtgji}{\dot{\tilde{g}}_{ji}}


% Node state differences
\newcommand{\xjmi}{x_j-x_i}
\newcommand{\vjmi}{v_j-v_i}
\newcommand{\nxjmi}{\norm{\xjmi}}

% Notation for desired quantities
\newcommand{\xgi}{x_{g,i}}
\newcommand{\xgj}{x_{g,j}}
\newcommand{\betagij}{\beta_{g,ij}}
\newcommand{\dgij}{d_{g,ij}}


==> preamble/graphicsExport.tex <==
% activate externalization of figures
\usetikzlibrary{external}
\usepackage{cprotect}

\tikzexternalize 

%command to insert a Beamer frame from a sketch and externalize with the same name 
\newcommand{\insertsketchframe}[2][.]{\section{$\mathrm{#2}$}%
\tikzsetnextfilename{#2}%
  \begin{tikzpicture}[scale=0.7]%
    \input{#1/sketch/#2}%
  \end{tikzpicture}%
\endpgfgraphicnamed%
}

%command to insert a Beamer frame from a tikz drawing and externalize with the same name 
\newcommand{\inserttikzframe}[2][.]{\section{$\mathrm{#2}$}%
\tikzsetnextfilename{#2}%
\input{#1/tikz/#2}%
\endpgfgraphicnamed%
}


==> preamble/math.tex <==
% AMS typesetting
\makeatletter
\@ifpackageloaded{amsmath}{}{%
\usepackage[cmex10]{amsmath}%
}
\makeatother
\usepackage{mathtools}
\usepackage{amssymb,amsfonts}
\makeatletter
\@ifundefined{proof}{%
\usepackage{amsthm}%
}{}
\makeatother
% Generic symbols (e.g., \degree)
\usepackage{gensymb}
% Prescripts, squashed summations, and others
\usepackage{mathtools}
% Bold greek letters
\usepackage{bm}

%Common math statements environments
\makeatletter
\@ifundefined{theorem}{
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{fact}{Fact}
\newtheorem{problem}{Problem}
\newtheorem{assumption}{Assumption}
\newtheorem{property}{Property}
\newtheorem{remark}{Remark}
}{}
  %SIAM article classes give their own Definition and Remark environments
\@ifundefined{definition}{
  \newtheorem{definition}{Definition}
}
% \@ifundefined{remark}{
%   \newtheorem{remark}{Remark}
% }
\makeatother
\newcommand{\rmss}[1]{_{\textrm{#1}}}

%%% Local Variables: 
%%% mode: latex
%%% End: 


==> preamble/posterCommon.tex <==
\input{preamble/posterGraphics}
\input{preamble/posterFormatting}

%%% Local Variables: 
%%% mode: latex
%%% End: 


==> preamble/posterFormatting.tex <==
%fonts
\usepackage[scaled=0.90]{helvet}
\usepackage{courier}

%sectioning
\pagestyle{empty}
\setcounter{secnumdepth}{0}

%headings
\def\Head#1{\noindent\hbox to \hsize{\hfil{\veryHuge\color{DarkBlue} #1}}\bigskip}
\def\LHead#1{\noindent{\LARGE\color{Blue} #1}\vspace{-.5cm}}
\def\Subhead#1{\noindent{\Large\color{DarkBlue} #1}\vspace{-.5cm}}
\def\Subsubhead#1{{\color{Blue} #1}}
\def\Title#1{\noindent{\Huge #1}}

%text boxes and grid
%Note: use options showboxes if you want to see the boxes
\usepackage[absolute]{textpos}
\TPGrid[30mm,30mm]{10}{20}  % 3 - 1 - 7 - 1 - 3 Columns

% Mess with these as you like
\parindent=0pt
%\parindent=1cm
\parskip=0.5\baselineskip


==> preamble/posterGraphics.tex <==
\usepackage{tikz}
\usepackage{xcolor}

%colors
\definecolor{Blue}{rgb}{0.05,0.2,0.5}
\definecolor{DarkBlue}{rgb}{0.1,0.1,0.5}
\definecolor{LightBlue}{rgb}{.2431,.5451,.8588}
\definecolor{Red}{rgb}{1.0,0,0}
\definecolor{LightGray}{rgb}{0.95,0.95,0.95}

%for callouts
\usetikzlibrary{calc,chains,positioning,shapes.callouts}

%bullet points
\renewcommand{\labelitemi}{\color{LightBlue}{$\bullet$}}

%highlighting
\newcommand{\alert}[1]{{\color{LightBlue} #1}}

%rounded boxes
\newenvironment{roundboxes}[1][]
{\begin{tikzpicture}[start chain,node distance=2cm,
 every node/.style={on chain, text=black,fill=LightBlue!20, rounded corners=0.6cm},#1]
}
{\end{tikzpicture}
}

%Define anchors for callouts
\newcommand{\anchor}[1]{\tikz[remember picture] \coordinate (#1);}

%Insert callouts. Syntax:
%\callout[optionalStyle]{pointer}{positionRelativeToThePointer}{text}
\newcommand{\callout}[4][]{\begin{tikzpicture}[remember picture, overlay]
 \node[rectangle callout, fill=gray!50, #1, callout absolute pointer={#2}] at ($ #2 + #3 $) {#4};
\end{tikzpicture}
}

%Rounded box to highlight plus define anchor
\newcommand{\enboxref}[3][]{
  \tikz[baseline,remember picture]{
    \node[fill=gray!20,anchor=base,rounded corners=0.6cm,#1] (#2) {#3};
  }
}

%Boxes to define sections
\newlength{\sectionboxpadding}
\setlength{\sectionboxpadding}{5mm}

\newcommand{\sectionboxcolor}{LightBlue}

\newcommand{\sectionboxstart}[1]{\makebox[0cm][l]{\anchor{#1 a}}}
\newcommand{\sectionboxend}[1]{\makebox[0cm][l]{\anchor{#1 b}} \vspace{-3em}\\}
\newcommand{\sectionboxdraw}[2][]{\begin{tikzpicture}[remember picture, overlay,#1]
 \draw[rounded corners, line width=5pt, draw=\sectionboxcolor] ($(#2 a)+(0,0.6em)+(-\sectionboxpadding,\sectionboxpadding)+(0,0.4em)$) rectangle ($(#2 b)+(\textwidth,1em)+(\sectionboxpadding,-\sectionboxpadding)+(0,0.4em)$);
\end{tikzpicture}
}

\newcommand{\generalboxdraw}{
\begin{tikzpicture}[remember picture, overlay, LightBlue]
\draw[line width=5pt] ($(current page.north west) + (2,-13.5)$) rectangle ($(current page.south east) + (-2,3)$);
\end{tikzpicture}
}


==> preamble/preambleHelp.tex <==
\section*{Markup and commenting commands}
Use the command \var{\textbackslash newcommenter\{cname\}\{color\}} to enable the following commands (substitute \var{cname} with your pseudonim of choice, e.g., \var{rtron}, and \var{color} with a color name supported by the \var{xcolor} package):
\begin{itemize}
\item \var{\textbackslash cname\{comment\}}: typeset a colored comment labeled with the pseudonim.
\item \var{\textbackslash atcname}: use this to refer to another commenter.
\item \var{\textbackslash cnamehl\{comment\}\{text\}}: use this to highligth a portion of the text and comment on it.
\end{itemize}
Examples after using \var{\textbackslash newcommenter\{rtron\}\{Green3\}}:
\begin{itemize}
\item \var{\textbackslash rtron\{Ignore this comment\}} produces \rtron{Ignore this comment}.
\item \var{\textbackslash atrtron} produces \atrtron.
\item \var{\textbackslash rtronhl\{Sentence is obvious\}\{The sky is blue\}} produces \rtronhl{Sentence is obvious}{The sky is blue}
\end{itemize}

Use the command \var{\textbackslash sout} to strike out text.

Use \var{\tikztestgrid{4}{3}} to draw, inside a \var{tikzpicture}, a test grid 4 units wide, 3 units tall, and centered at (0,0).

==> preamble/proposals.tex <==

\input{preamble/compactLists}
\input{preamble/proposalsPagination}
\input{preamble/proposalsFormatting}
\input{preamble/splitting}

\newcommand{\testgrid}{\tikz[remember picture, overlay]{%
  \coordinate (tl) at  ($(current page.north west)+(1in,-1in)$);%
  \coordinate (br) at  ($(current page.south east)+(-1in,1in)$);%
  \draw[red] (tl) rectangle (br);%
  \draw[red] (tl) grid[xstep=2\textwidth,ystep=1in] (br);}}




==> preamble/proposalsAggressive.tex <==
\linespread{0.93}


==> preamble/proposalsEnableHelvetica.tex <==
%These commands set Helvetica as the default font
\usepackage[scaled]{helvet}
\renewcommand\familydefault{\sfdefault} 
\usepackage[T1]{fontenc}


==> preamble/proposalsFormatting.tex <==

\paragraphswithstop 

% Reduce line skip before \paragraph
\titlespacing{\paragraph}{%
  0pt}{%              left margin
  0\baselineskip}{%   space before (vertical)
  0.5em}%             space after (horizontal)


% Change name of section for references
\renewcommand{\refname}{References Cited}

%Redefine \maketitle command
\makeatletter
\renewcommand{\maketitle}{\begin{center}\Large\textbf\@title
  \end{center}
  % Add author only if not empty (in the sense of producing output)
\setbox0=\hbox{\@author\unskip}\ifdim\wd0=0pt
\else
\begin{center}
  \@author
\end{center}
\fi%
}
\makeatother

%theorem-like environment for stating thrusts
%we define a second counter that is updated in synch with the default
%one, but is presented in Alphabetic form
\newtheorem{innerthrust}{Thrust}
\newcounter{thrustnumber}
\newenvironment{thrust}[1][\Alph{thrustnumber}]
  {\stepcounter{thrustnumber}\renewcommand\theinnerthrust{#1}\innerthrust}
  {\endinnerthrust}


%macros for paragraphs in thrust description
\newcommand{\thrustmerits}{\paragraph{Intellectual merits of
    this thrust}}
\WithSuffix\newcommand\thrustmerits*[1][\Alph{thrustnumber}]{\paragraph{Intellectual merits of thrust~#1}}

\newcommand{\thruststateoftheart}{\paragraph{State of
    the art and open problems}}
\WithSuffix\newcommand\thruststateoftheart*[1][\Alph{thrustnumber}]{\paragraph{Relation of thrust~#1 with the state of the art}}

\newcommand{\thrustbackground}[1]{\paragraph{Background on #1}}

\newcommand{\thrustgoal}{\paragraph{Goal of this thrust}}

\newcommand{\proposalcontribution}[1]{\paragraph{Proposed innovation: #1}}

\newcommand{\collaborationletter}{\emph{Letter of collaboration}}

\setlist[description]{%
  font={\itshape}, % set the label font
}

\newenvironment{wrapremark}[2][]
{  \setlength{\intextsep}{0em}
  \wrapfigure{#2}{0.4\textwidth}\vspace{-0.5em}\mdframed\vspace{-3mm}\remark[#1]}
{\endremark\endmdframed\endwrapfigure}



==> preamble/proposalsNIH.tex <==
\input{preamble/proposalsEnableHelvetica}
\geometry{margin=0.5in}

==> preamble/proposalsPagination.tex <==
\usepackage{url}
\usepackage{times}

\usepackage[compact]{titlesec}

% Perfect 1 inch margins
\usepackage[letterpaper,margin=1in]{geometry}

%Make font for captions smaller (saves space and visually separates them from the main text)
\usepackage[font={footnotesize,sf}]{caption}

% Nice gantt charts
\usepackage{pgfgantt}



==> preamble/proposalsTaskSections.tex <==
%The following reformat the sections so that their labels read "Task x.y" instead of "x.y".
%Use the starred version of the command if you do not want this for
%some of the sections
\titleformat{\section}{\normalfont\large\bfseries}{Task \thesection:}{0.5ex}{}
\titleformat{\subsection}{\normalfont\bfseries}{Task \thesubsection:}{0.5ex}{}


==> preamble/proposalsTitles.tex <==
%Common style that will be used for titles
\newcommand{\titlestyle}{\color{DodgerBlue4}\sffamily}

%Format titles
\titleformat*{\section}{\titlestyle \bfseries \Large}
\titleformat*{\subsection}{\titlestyle \bfseries \large}

%Lists (requires enumitem package):
%Font for description
\setlist[description]{font=\color{DodgerBlue3}}
%Compact lists
\setlist[1]{\labelindent=\parindent}
\setlist[1]{topsep=3pt, itemsep=0pt}

%Format main title
\let\prevtitle\title
\renewcommand{\title}[1]{\prevtitle{\titlestyle #1}}
\let\prevauthor\author
\renewcommand{\author}[1]{\prevauthor{\titlestyle #1}}
\let\prevdate\date
\renewcommand{\date}[1]{\prevdate{\titlestyle #1}}
\renewcommand{\paragraph}[1]{\par\noindent{\titlestyle\small\bfseries #1.~}}

% Format mdframed boxes
\mdfsetup{%
  middlelinecolor=DodgerBlue4,
  middlelinewidth=1pt,
  %backgroundcolor=red!10,
  roundcorner=3pt}

==> preamble/roboticsHelp.tex <==
This file introduces commands for drawing axes and cameras.

\begin{itemize}
\item \var{ax[label][opts]\{refid\}\{x\}\{y\}\{rot\}} Draws a pair of 2-D axes. \var{refid} can be the used to put labels and third axes.
\item \var{axup[label_rotation]\{refid\}\{label\}\{rot\}}
\item \var{axlabels\{refid\}\{label1\}\{label2\}}
\item \var{camera[label]\{refid\}\{x\}\{y\}\{rot\}}
\item \var{gpoint\{coordinates\}\{label\}\{rot\}}
\end{itemize}


==> preamble/splitting.tex <==
%Macro to include file while writing to log file the splitting markers
\newenvironment{markforsplit}[1]{%
  \def\splitmarkername{#1}
  \typeout{Split marker [#1] [start] [\theCurrentPage]}  \setcounter{page}{1}%
  \setcounter{figure}{0}%
  \setcounter{table}{0}%
}{%
  \clearpage%
  \typeout{Split marker [\splitmarkername] [end] [\theCurrentPage]}%
}
\newcommand{\includeforsplit}[1]{%
\begin{markforsplit}{#1}%
\include{#1}%
\end{markforsplit}%
}

